Approximate Cluster-Based Sparse Document Retrieval with Segmented Maximum Term Weights

This paper revisits cluster-based retrieval that partitions the inverted index into multiple groups and skips the index partially at cluster and document levels during online inference using a learned sparse representation. It proposes an approximate search scheme with two parameters to control the rank-safeness competitiveness of pruning with segmented maximum term weights within each cluster. Cluster-level maximum weight segmentation allows an improvement in the rank score bound estimation and threshold-based pruning to be approximately adaptive to bound estimation tightness, resulting in better relevance and efficiency. The experiments with MS MARCO passage ranking and BEIR datasets demonstrate the usefulness of the proposed scheme with a comparison to the baselines. This paper presents the design of this approximate retrieval scheme with rank-safeness analysis, compares clustering and segmentation options, and reports evaluation results.

==> emnlpclust.tex <==

\subsection{Segmentation choices}
\label{sect:clustering}

\comments{
We first discuss how to cluster   documents. 
Here, we assume that  a learned sparse representation is produced from a trained  transformer encoder $T$. For example, 
SPLADE~\cite{Formal2021SPLADE, Formal_etal_SIGIR2022_splade++} and LexMAE~\cite{shen2023lexmae} provide a trained
BERT transformer to encode a document and a query.
%After  training, such a  model produces  a transformer encoder $T$ which can be used to 
%produce a weight vector for each document in a data collection.  
There are two approaches to represent documents for clustering:
% using a learned sparse representation. 


\begin{itemize} [leftmargin=*]
\item {\bf K-means clustering of sparse vectors.} 
Encoder $T$  is applied  to each document in a data collection  
to produce a sparse weighted  vector. 
Similar as Anytime Ranking~\cite{2022ACMTransAnytime},
we follow the approach of ~\cite{2015ACMTrans-KulkarniCluster, 2017InfoRetrJ-KimSelective} 
to apply the  Lloyd's k-means clustering~\cite{k-means}. 
Naively applying the k-means algorithm to the clustering of learned sparse vectors presents a challenge
owing to their high dimensionality and a large number of sparse vectors as the dataset size scales. 
%to sparse document vectors produced by the given neural retrieval model.
%There is a weakness with sparse clustering that the dimensionality of learned  sparse vectors is large.
For example, each sparse SPLADE document vector is  of  dimension 30,522 although  most  elements are zero.
Despite its efficacy and widespread use, the k-means algorithm is known to deteriorate when the dimensionality grows.
Previous work on sparse k-means has addressed that  with feature selection and 
dimension reduction~\cite{2020NEURIPS-kmeans, 2020IJCAIkmeans}.
These studies explored dataset sizes much smaller than our context and with different applications. 
Thus our retrieval application demands new considerations. 
%The above techniques have not been investigated in the context of sparse retrieval, and
%the impact of thresholding  on relevance and query processing time with inverted indices,
%requires new design considerations and model structuring for document retrieval, even the previous work can be leveraged.
Another difficulty is a lack of efficient implementations for sparse k-means in dealing with large datasets. 
%It is computationally complex and expensive  to scale k-meaning to deal with  a large number of sparse vectors of a high dimenality.
We address the above  challenge below by taking advantage of  the dense vector representation produced by the transformer encoder
as counterparts corresponding to their sparse vectors,  with a much smaller dimensionality.  

\item {\bf K-means clustering of dense vector counterparts.} 
%We produce a dense vector for each document using the neural transformer trained with the sparse retriever model.
Assuming this trained transformer $T$ is BERT, we apply $T$ to each document and produce 
a token embedding set $\{t_1, t_2, \cdots, t_L\}$ and  a CLS token vector.
Here $t_i$ is  the BERT output embedding of $i$-th token in this document
and $L$ is the total number of tokens of this document. Then, we have three ways to produce a dense vector of each document for clustering.
\begin{itemize}
\item The CLS token vector.
\item The element-wise maximum pooling of  all output 
token vectors.  The $i$-th entry of this dense vector is $\max_{j=1}^L t_{i,j}$ where $t_{i,j}$ is the $i$-th entry of $j$-th token embedding.
\item The element-wise mean pooling of all output
 token vectors. The $i$-th entry of this dense vector 
is $\frac{1}{L} \sum_{j=1}^L t_{i,j}$ where $t_{i,j}$ is the $i$-th entry of $j$-th token embedding.
\end{itemize} 
In addition to the above options, we have compared the use of a dense representation 
based on SimLM~\cite{Wang2022SimLM},  a state-of-the-art dense retrieval model. 
 
\end{itemize} 
BERT vectors are of  dimension 768, and   we leverage the FAISS library~\cite{johnson2019billion} 
for dense vector clustering with quantization support, 
which can compress vectors and further reduce the dimensionality.

%\subsection{Impact of different clustering methods}

\input{tables/cluster_method}
Table~\ref{tab:clustering}  compares  the performance of ASC in a safe mode $(\mu=\eta=1)$
using the above five different vector representation options to  apply k-means  clustering
for  SPLADE-based sparse  retrieval.
There are 4096 clusters and eight random segments per cluster.
MRT is the mean retrieval time in milliseconds. 
Column marked with ``\%C''  shows the percentage of clusters that are not pruned during ASC retrieval.
\comments{
We compare the following options with k-means clustering: 
1) dense CLS token vectors generated using the BERT transformer trained in the SPLADE model;
2) average dense  vector  of document tokens transformed  using BERT;
3) sparse document  vectors  encoded using SPLADE.
The above options without segmentation are compared against
}
%The maximum pooling method  listed in this table uses  two options:  with and without segmentation.
For sparse vectors, we leverage FAISS dense k-means implementation with sampling, which is still expensive.
Table~\ref{tab:clustering}  
shows that the maximum pooling of SPLADE-based dense token vectors has a similar latency as the sparse vector representation. 
These two options are better than other three options.
Considering the accuracy and implementation challenge in clustering   high-dimension sparse vectors, our evaluation chooses
max-pooled dense vectors derived from the corresponding transformer model.
%skips the most clusters and gives the shortest latency.
%That is the reason that this maximum pooling with k-means clustering is used in our evaluation.
%in Tables~\ref{tab:msmarco} and \ref{tab:beir}.  




%We find that the k-means clustering applied to the dense vector with maximum pooling  
%yields the best solution for ACS.

{\bf Cluster segmentation methods for weight information  collection.} 
}
There are two approaches to subdivide each cluster for
segmented term weights   during offline processing. 
%Notice the inverted index for each cluster is not subdivided during online inference while segmented weight information  per  cluster 
%is stored for online access
\begin{itemize} [leftmargin=*]
\item {\bf Random uniform partitioning}.
This random partitioning
allows ASC to satisfy the probabilistic safeness condition that
each document in a  cluster has an equal chance to appear in any segment.

\item {\bf K-means sub-clustering}.
This is to use the same  clustering for partitioning the entire dataset based on document similarity.
As shown below, this method turns out to be less  effective than random uniform partitioning.
\end{itemize} 


\comments{
{\bf Data needed.}
\begin{itemize}
\item 1) X-axis: a few settings varying  the number of clusters or other configurations.\\
Y-axis:  the average error sum or squared error between document rank score and cluster upperbound under different clustering methods.\\
Y-axis: Latency and relevance of our algorithm under different clustering methods.\\
\item 2) Impact on upperbound estimation error, latency, and relevance of using different segmentation: random partitioning vs K-mean subclustering.
\end{itemize}
}


\input{tables/rand_vs_kmeans}

The top portion of Table~\ref{tab:segmentrandom} compares the above two segmentation methods
when applying SPLADE to MS MARCO passages with 4098 clusters and 8 segments per cluster.
% The random segmentation offers better MRR@10 number and recall@1k especially when $\mu$ varies from 0.3 to 1 and $\eta$ is fixed to be 1.
%Columns 2 and 3  are for k-means subclustering while Columns 4 and 5  are for random partitoning.
Random uniform partitioning 
%, matching the condition of  Proposition~\ref{propsafe2},
offers equal or better relevance in terms of MRR@10 and Recall@1000, especially when $\mu$ is small.
As $\mu$ affects cluster-level pruning in ASC, random segmentation results in a better prevention of incorrect  aggressive pruning, although 
this can result in less cluster-level pruning and a longer latency. 
% because random segmentation allows any document in a cluster has an equal chance to appear in any segment of this cluster.
%whilt its latency is relatively larger than k-means subclustering.
To provide an explanation for  the above result, 
the lower portion of Table~\ref{tab:segmentrandom} 
shows the average ratio of actual cluster upper bound over the estimated $MaxSBound$,
and the average difference of $MaxSBound$ and $AvgSBound$ scaled by the actual bound.
%when the segmentation uses random and uniform paritioning  and   k-means subclustering.
Random uniform partitioning provides slightly better cluster upper bound estimation,
while its average difference of $MaxSBound$ and $AvgSBound$ is much smaller than  k-means sub-clustering.
Then, when $\mu$ is small, there are more un-skipped clusters, following Proposition~\ref{prop:avgprune}.
 
%Thus, random segmentation yields more accurate bound estimation and triggers   less cluster-level pruning, while being relatively slower when $\mu \leq 0.5$.
The above result also indicates  cluster-level pruning in ASC becomes safer due to its adaptiveness to
the gap between the maximum and average segment bounds, which is  consistent with   Proposition~\ref{prop:avgprune}.
The advantage of random uniform partitioning  shown above corroborates with Proposition~\ref{propsafe2} and
demonstrates the usefulness of   possessing  probabilistic approximate rank-safeness. 
%We provide more evaluation results in the next section.  

\comments{
{\bf Observations.}
\begin{itemize}
\item K-means partitioning can be faster if $mu$ is set low, since its $AvgSBound$ is tighter, thus more clusters can be pruned. As a result, its relevance drops more when  $mu$ gets smaller.
\item With random partitioning, setting $eta=1$ yields reasonably good relevance no matter how small $mu$ is, reflecting Proposition \ref{propsafe2}.

\end{itemize}
}


==> emnlpintro.tex <==
\section{Introduction}

There are two categories of approaches for top $k$ search of text documents. 
One  category is transformer-based dense retrieval with 
dual encoders (e.g.  ~\cite{Karpukhin2020DPR
Ren2021RocketQAv2,Liu2022RetroMAE, Zhang2022AR2, Wang2022SimLM}),
and this approach gains its popularity due  to its ranking model simplicity based 
on dot products which can  take  advantage of GPU availability for fast computation.
%through negative example sampling, model dstillation, and  pretraining optimization.  
Another category is 
%expensive and time-consuming cross-encoders to achieve %impressive MRR score 0.437 and 0.419, respectively,  for MS MARCO passage ranking.  
%impressive MRR score (up-to 0.437)  
classical retrieval methods for  document search use  an 
inverted index to match documents with additive ranking such as BM25~\cite{Robertson2009BM25},
taking advantage of the inverted index implementation to deliver fast dot products on CPUs.
This method gains its popularity in last few years due to the advancement of  learned sparse representation
which  exploits transformer-based neural models to learn document tokens with neural 
weights~\cite{Dai2020deepct, Mallia2021deepimpact, Lin2021unicoil,2021NAACL-Gao-COIL,
Formal2021SPLADE, Formal2021SPLADEV2,Formal_etal_SIGIR2022_splade++, shen2023lexmae}.
For the standard ranking test data  with MS MARCO passages, 
relevance numbers accomplished by these two categories  are comparable with a well-trained model.
For the standard zero-short retrieval tests with BEIR datasets, learned sparse retreival exhibits better performance than 
BERT-based dense models.
While GPUs are readily available, they are very  expensive and require much more energy consumption than CPUs.
For example, AWS EC2 charges  one or two order of magnitude more  
for an advanced  GPU (e.g. p3dn.24xlarge) than a CPU with similar memory capacity (e.g. x2gd.4xlarge).   
%(p3dn.24xlarge vs x2gd.4xlarge).   
%per hour for this GPU than CPU based on their published cost table
\comments{
For a large-scale high-query-traffic search platform such as Google or Bing,
GPUs are appropropriate for innitial query process and final ranking at the later stage of processing
pipeline. But they are not   attractive for first-stage retrieval because such a system divides the 
large index into many partitions and runs searches with replication on tens of thousands of machines in parallel 
within a data center. Will multi-data center replications, deploying GPUs in first-stage retrieval would easily incur 
billions of dollars more  and consume an order of maganute more energy.
}

%In last few years,
%with an advancement of neural information retrieval, 
% SNRM ~\cite{Zamani2018SNRM},
%DeepCT~\cite{Dai2020deepct}, DeepImpact~\cite{Mallia2021deepimpact}, uniCOIL~\cite{Lin2021unicoil,2021NAACL-Gao-COIL},
%and SPLADE~\cite{ Formal2021SPLADE, Formal2021SPLADEV2,Formal_etal_SIGIR2022_splade++}
%Formal2021SPLADE, Formal2021SPLADEV2, Mallia2021deepimpact, Lin2021unicoil.   Bai2020SparTerm, 
%As a standard reference point, we will use the popular
%A popular  method called BM25 uses a linear additive scoring based on term frequency~\citep{Robertson2009BM25} to retrieve top results before re-ranking.
%and can  take advantage of traditional inverted index based retrieval techniques~\cite{Mallia2017VBMW,mallia2022faster}. 
% for fast retrieval from a large dataset  on a CPU-only platform
%Learned sparse retrieval methods can be effective in relevance on average for in-domain and out-of-domain search  compared  to 
%BERT-based dense retrieval with dual encoders (e.g. ~\cite{Ren2021RocketQAv2,Santhanam2021ColBERTv2,Liu2022RetroMAE}).
%Its query processing is relatively cheap and fast  without GPU support, by taking advantages of  sparse  inverted indices,

%specially with index and  model  
%optimization ~\cite{2022EMNLP-mackenzie-clipping, lassance2022efficiency,mallia2022faster,20232GT,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning}.
%Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning
%While dense retrieval is an active topic of research taking advanges of pretrained 
%language models even with efficiency optimization  through approximate nearest neighbor  search~\cite{johnson2019billion, 2022WSDM-Zhan-RepCONC, Xiao2022Distill-VQ}.
This paper is focused on online inference efficiency optimiation for sparse representations.
Traditional optimization to speed up top-$k$ sparse retrieval given an inverted index is through dynamic pruning techniques,
such as MaxScore~\cite{Turtle1995}, WAND~\cite{WAND}, and BlockMax WAND (BMW)~\cite{BMW}
which  safely skip the evaluation of low-scoring documents that are unable to appear in the final top-$k$ results.
Anytime Ranking by Mackenzie et al.~\cite{2022ACMTransAnytime}
extends the  earlier cluster-based retrieval studies~\cite{2017ECIR-SelectiveSearch,2004InfoJ-ClusterRetr}
to organize the inverted index as clusters with ranges of document IDs,
% and selects clusters
and  dynamically prune clusters under a time budget.
Such early search termination with a budget can be viewed as a  category of ``rank-unsafe'' pruning. 
There is another line of work on dynamic unsafe pruning called threshold 
over-estimation~\cite{2012SIGIR-SafeThreshold-Macdonald, 2013WSDM-SafeThreshold-Macdonald, 2017WSDM-DAAT-SAAT} and it is
a focus of this paper.
%Unsafe pruning with threshold estimation is considered earlier in ~\cite{2019CIKMYafay, 2019SIGIR-Petri, TwoTierBMW}. 

%Considering the above advancement  of sparse retrieval with learned representations, 
This paper  revisits  dynamic  index pruning in both safe and  unsafe aspects in the context of cluster-based retrieval. 
Our approach combines cluster-based retrieval with threshold over-estimation and improves its pruning safeness for better relevance effectiveness
or being faster  while retaining the same level of relevance. 
%through probabilistically safeness competitive in safeness .  
%The focus of this paper is to accelerate cluster-based retrieval with threshold-driven  pruning.
Specifically, the contributions of this paper are listed as follows:
%to propose and evaluate the following techniques:
% to accelerate  cluster-based sparse index traversal: 
%\begin{itemize} [leftmargin=*]
%\item Selective cluster revisiting to reduce  search approximation error with a second chance.
%\end{itemize} 


\begin{itemize} [leftmargin=*]
\item 
%Tighter  cluster-level   rank score bound estimation increases the likelihood to
We propose cluster-level  maximum weight segmentation that partitions a cluster 
into segments offline and  collects segmented term weight information.
This allows cluster-based retrieval to tighten  rank score bound estimation and accurately 
skip more  clusters that only contains low-scoring documents. 
%degree of cluster-level rank score upper bounds duing online inference.

%\item Cluster-level  maximum term weight segmentation 
%to improve the estimation tightness of document rank score upperbounds  within each cluster, which allows more safe skipping.
%two control parameters.
%Our first idea is to improve the accuracy of upper bound estimation using cluster segmentation.
%When similar documents are subgrouped, their upperbound estimation can become more accurate.
%An alternative method to divide documents into many clusters to improve bound estimation, and having  a large number of clusters, however,
%incurs more overhead and decreaes the effectiveness of MaxScore index pruning.

\item We analyze the rank-safeness approximation property of threshold over-estimation and 
propose a two-parameter pruning control to provide  a probabilistic approximate rank-safeness  guarantee. 
This control utilizes   randomly-segmented maximum term weights, and  
makes  cluster-level pruning  approximately adaptive  to  the bound estimation tightness for improved safeness. 
%In this context, we also provide an analysis   on the benefit of 
%While we use the upper bound estimation to guide the selection of clusters, we have also incorporated the
%to guide the selection of sparse document vector clusters.
%\item Faster search with threshold over-estimation and safer cluster pruning by 
%and with an approximate and probabilistic safeness  assurance by exploiting  randomly segmented cluster information.

\comments{
\item
%Clustering of many sparse vectors of a high dimensionality is not easy and
We exploit the use of dense token embeddings as counterparts of sparse vectors under the SPLADE-like models~\cite{Formal2021SPLADE,shen2023lexmae} 
 to cluster documents with k-means and  support the above scheme. 
%\item 
%A comparison of different document representation options  for k-means clustering and an 
%An exploitation of dense vectors corresponding
%to  sparse vectors built on the top of a SPLADE-like neural model
%to cluster documents with k-means and
\item We conduct extensive  evaluations  on    the MS MARCO and BEIR datasets to validate the effectiveness of 
the proposed scheme, called {\bf ASC}. 
This paper  demonstrates  the use of ASC with three  learned sparse retrieval models:
SPLADE~\cite{Formal2021SPLADE,Formal_etal_SIGIR2022_splade++}, uniCOIL~\cite{Lin2021unicoil,2021NAACL-Gao-COIL}, and LexMAE~\cite{shen2023lexmae}.
We  study  its benefit when used with   
two orthogonal efficiency  optimization techniques:  anytime early termination~\cite{2022ACMTransAnytime}
and static index pruning~\cite{2023SIGIR-Qiao}.
%is complementary to the orthogonal efficiency  optimization techniques for learned sparse retrieval 
%~\cite{2022EMNLP-mackenzie-clipping, Lassance2022SPLADE-efficient,mallia2022faster,qiao2023optimizing,2023SIGIR-Qiao, 2023SIGIR-SPLADE-pruning} and
}
\end{itemize}

We conduct extensive  evaluations  on    the MS MARCO and BEIR datasets to validate the effectiveness of 
the proposed scheme, called {\bf ASC}. 
This paper  demonstrates  the use of ASC with three  learned sparse retrieval models.





==> graph.tex <==
\subsection{Second-chance revisiting of skipped clusters}
\label{sect:revisit}

After execution of ACS to conduct cluster-based  $(\mu, \eta)$-approximate  retrieval  with segmentation,
there exists a chance that good clusters may be skipped when ASC is configured with $\mu <1$.
To reduce the chance of  missing important documents, we give a second chance to each skipped cluster and 
conduct another phase of selective visitation for skipped clusters
by inspecting the similarity-based neighbor clusters of top documents retrieved so far.
The key idea is to examine if some content of a skipped cluster is similar to the clusters containing top ranked documents retrieved by ASC.
When ASC is combined together with this selective cluster revisiting for the second chance, we call it ASC2. 

The detail of this second chance  method is summarized as follows.
\begin{itemize} [leftmargin=*]
\item {\bf Derivation of document-to-cluster similarity links.} During cluster index generation, we also keep top $n$ neighbor clusters  of each document $x$.
A  neighbor cluster is the one that contains  document $y$ similar to  $x$.
The top $n$ document neighbors of $x$ are found by using the document text of $x$ as a query to search the inverted index of the dataset.

\item {\bf Second-chance priority computation  of skipped clusters.}
After the first ASC retrieval phase, we derive  the cluster distribution of the top $k'$ results retrieved so far
and  computer the similarity of a skipped cluster $C$ to the top cluster
as the weighted count of top $k'$ documents  contained in cluster $C$. 
This value is used in the next step as  the priority of each skipped cluster. 

\item {\bf Sparse retrieval on selected clusters.}
We select top $m$ skipped clusters based on their priority defined in the above step.
Then we conduct sparse retrieval on these top $m$ clusters to supplement the result of ASC.  
\end{itemize} 

{\bf Online space overhead.}  The second-chance priority requires an added space cost 
to host the document-to-cluster similarity links.
We find in our evaluation that a low double digit number of neighbors for each document is sufficient for similarity driven cluster selection.
For example, in MS MARCO, 20 neighbors are sufficient.
With $v$ documents,  each document keeps top $n$ neighbor links to clusters.  assume 2 bytes are sufficient to represent cluster IDs.
The total space cost is $40v$ bytes. With $v=8.8$ million pages in MS MARCO, the total space cost is 352MBbytes.

Selective dense retrieval in ~\cite{2020TPAMI-HNSW, 2022CIKM-MacAvaneyGraphReRank,  2023SIGIR-LADR}.
uses   document-to-document similarity to select dense embeddings.  
A key difference is that we  use  document-to-cluster similarity in a new context for  second-chance sparse cluster revisiting. 

\comments{
{\bf Data needed.}
\begin{itemize}
\item X-axis: a few settings varying  the number of clusters or other configurations (different neighbors).\\
Y-axis: Latency and relevance of our algorithm with and without graph.\\
\end{itemize}

}


==> tables/cluster_size.tex <==
\begin{table}[htbp]

% \footnotesize
    \centering
        \caption{SPLADE-Cluster performance on MS MARCO (SPLADE-Dense-Max)}
\label{tab:segmentation}
\resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{l|cc|cc}
    \hline
     \textbf{Methods} & \textbf{MRR, R} & \textbf{MRT} & \textbf{Docs Visited} & \textbf{Cluster Size} \\ 
    \hline
    % SPLADE & 0.3940 & 121(483) & 278(819) & 23.3 & 312  \\
    % SPLADE*-(40)50 & 0.3906- & - & - \\
    % SPLADE*-(60)70 & 0.3839- & - & - \\
    w/o sub. (safe) & 0.3966, 0.9802 & 90.0 & 68\% & 4096 \\
    w/ sub. (safe) & 0.3966, 0.9802 & 70.1 & 54\% & (4096 $\times$ 8) \\
    w/ sub. (unsafe) & 0.3941, 0.9475 & 14.0 & 4.5\% & (4096 $\times$ 8) \\
    \hline
    w/ sub. (safe) & 0.3966, 0.9802 & 49.7 & 74\% & (1024 $\times$ 32) \\
    w/ sub. (unsafe) & 0.3937, ?? & 20.3 & 12\% & (1024 $\times$ 32) \\
    \hline
     
    \end{tabular}
   }
\end{table}


==> tables/graph.tex <==
\begin{table}[htbp]

% \footnotesize
    \centering
        \caption{(-Graph) performance on MS MARCO (SPLADE-Dense-Max), 4096 $\times$ 8}
\label{tab:graph}
\resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{l|cc|c}
    \hline
     \textbf{$\mu$, $\eta$, $\#G$, $\#G_e$} & \textbf{MRR, R} & \textbf{MRT} & \textbf{Docs Visited} \\ 
    \hline
    % SPLADE & 0.3940 & 121(483) & 278(819) & 23.3 & 312  \\
    % SPLADE*-(40)50 & 0.3906- & - & - \\
    % SPLADE*-(60)70 & 0.3839- & - & - \\
    0.5, 1, 0, NA & 0.3954, 0.9588 & 17.7 & 6.4\%  \\
    0.5, 1, 20, 100 & 0.3959, 0.9700 & 19.9 & 6.8\%  \\
    0.5, 1, 20, 50 & 0.3962, 0.9702 & 19.5 & 6.8\%  \\
    0.5, 1, 20, 20 & 0.3963, 0.9703 & 19.0 & 6.8\%  \\
    0.2, 0.8, 20, 100 & 0.3890, 0.9296 & 9.3 &  \\
    0.2, 0.8, 50, 100 & 0.3915, 0.9435 & 11.0 &  \\
    0.2, 0.8, 50, 50 & 0.3913, 0.9428 & 10.8 &  \\
    0.2, 0.8, 50, 20 & 0.3914, 0.9426 & 10.6 &  \\
    0.2, 0.8, 50, 10 & 0.3912, 0.9417 & 10.5 &  \\
    \hline
     
    \end{tabular}
   }
\end{table}


==> tables/mu_eta.tex <==
\begin{table}[htbp]

% \footnotesize
    \centering
        \caption{SPLADE-Cluster(-Graph) performance on MS MARCO (SPLADE-Dense-Max), 4096 $\times$ 8}
\label{tab:mueta}

\resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{l|cc|c}
    \hline
     \textbf{$\mu$, $\eta$, $\#G$} & \textbf{MRR, R} & \textbf{MRT} & \textbf{Docs Visited} \\ 
    \hline
    % SPLADE & 0.3940 & 121(483) & 278(819) & 23.3 & 312  \\
    % SPLADE*-(40)50 & 0.3906- & - & - \\
    % SPLADE*-(60)70 & 0.3839- & - & - \\
    1, NA, 0 & 0.3966, 0.9802 & 70 & 54\%  \\
    0.6, NA, 0 & 0.3964, ?? & 29 & 14\%  \\
    0.5, NA, 0 & 0.3914, ?? & 16 & 5.7\%  \\
    0.5, 1, 0 & 0.3954, ?? & 18 & 6.4\%  \\
    0.45, 1, 0 & 0.3941, 0.9475 & 14 & 4.5\%  \\
    0.3, 0.9, 0 & 0.3892, 0.9168 & 10.1 &   \\
    0.3, 0.9, 15 & 0.3924, ?? & 11.2 &  \\
    0.3, 0.9, 30 & 0.3932, ?? & 12.0 &  \\
    0.3, 0.9, 50 & 0.3941, 0.9552 & 12.8 &  \\
    \hline
     
    \end{tabular}
   }
\end{table}

